COSMIC: COmmonSense knowledge for eMotion Identification in Conversations

In this paper, we address the task of utterance level emotion recognition in conversations using commonsense knowledge. We propose COSMIC, a new framework that incorporates different elements of commonsense such as mental states, events, and causal relations, and build upon them to learn interactions between interlocutors participating in a conversation. Current state-of-the-art methods often encounter difficulties in context propagation, emotion shift detection, and differentiating between related emotion classes. By learning distinct commonsense representations, COSMIC addresses these challenges and achieves new state-of-the-art results for emotion recognition on four different benchmark conversational datasets. Our code is available at https://github.com/declare-lab/conv-emotion.

==> old_tables.tex <==
\begin{table*}[ht]
  \centering
  \resizebox{\linewidth}{!}{
  % \tabcolsep=3pt
   \begin{tabular}{l||c@{~~}cc@{~~}cc@{~~}cc@{~~}||cc@{~~}cc@{~~}cc@{~~}c}
    \hline
    \multirow{2}{*}{Methods} & \multicolumn{7}{c||}{IEMOCAP} & \multicolumn{7}{c}{DailyDialog} \\
    \cline{2-15} & Happy & Sad & Neutral & Angry & Excited & Frustrated & \textbf{Avg(w)} & Happy & Angry & Sad & Fear & Surprise & Disgust & \textbf{Avg(m)}\\
    \hline
    \hline
    CNN & 29.86 & 53.83 & 40.14 & 52.44 & 50.09 & 55.75 & 48.18 & - & - & - & - & - & - & -\\
    Memnet & 33.53 & 61.77 & 52.84 & 55.39 & 58.30 & 59.00 & 55.10 & - & - & - & - & - & - & -\\
    bc-LSTM & 34.43 & 60.87 & 51.81 & 56.73 & 57.95 & 58.92 & 54.95 & - & - & - & - & - & - & -\\
    bc-LSTM+Att & 35.63 & 62.90 & 53.00 & 59.24 & 58.85 & 59.41 & 56.19 & - & - & - & - & - & - & -\\
    CMN & 30.38 & 62.41 & 52.39 & 59.83 & 60.25 & 60.69 & 56.13 & - & - & - & - & - & - & -\\
    ICON & 29.91 & 64.57 & 57.38 & 63.04 & 63.42 & 60.81 & 58.54 & - & - & - & - & - & - & -\\
    DialogueRNN & 33.18 & 78.80 & 59.21 & 65.28 & 71.86 & 58.91 & 62.75 & - & - & - & - & - & - & 40.3\\
    DialogueGCN & 42.75 & 84.54 & 63.54 & 64.19 & 63.08 & 66.99 & 64.18 & - & - & - & - & - & - & -\\
    DCR-Net & - & - & - & - & - & - & - & - & - & - & - & - & - & 48.9\\
    \hline
    CommonsenseRNN & \textbf{59.65} & 80.08 & \textbf{64.19} & \textbf{66.48} & 67.33 & 61.97 & \textbf{66.48} & 63.69 & 41.35 & 45.28 & 40.00 & 45.28 & 30.00 & \textbf{51.05}\\
    \hline
   \end{tabular}
  }
  \caption{Comparison with the baseline methods on IEMOCAP and DailyDialog dataset. Reported scores are F1 scores. Average(w) = Weighted average, Average(m) = Macro average.\label{tab:results1}}
\end{table*}


\begin{table*}[h]
  \centering
  \resizebox{\linewidth}{!}{
  % \tabcolsep=3pt
   \begin{tabular}{l||c@{~~}cc@{~~}cc@{~~}cc@{~~}||cc@{~~}cc@{~~}cc@{~~}c}
    \hline
    \multirow{2}{*}{Methods} & \multicolumn{7}{c||}{MELD} & \multicolumn{7}{c}{EmoryNLP} \\
    \cline{2-15} & Joy & Sad & Neutral & Angry & Excited & Frustrated & \textbf{Avg(w)} & Happy & Angry & Sad & Fear & Surprise & Disgust & \textbf{Avg(m)}\\
    \hline
    \hline
    CNN & - & - & - & - & - & - & 55.02 & - & - & - & - & - & - & -\\
    bc-LSTM & - & - & - & - & - & - & 56.44 & - & - & - & - & - & - & -\\
    bc-LSTM+Att & - & - & - & - & - & - & 56.70 & - & - & - & - & - & - & -\\
    DialogueRNN & - & - & - & - & - & - & 57.03 & - & - & - & - & - & - & -\\
    DialogueGCN & - & - & - & - & - & - & 58.10 & - & - & - & - & - & - & -\\
    \hline
    CommonsenseRNN &  &  &  &  &  &  & \textbf{65.84} &  &  &  &  &  &  & \\
    \hline
   \end{tabular}
  }
  \caption{Comparison with the baseline methods on MELD and EmoryNLP dataset. Reported scores are F1 scores. Average(w) = Weighted average, Average(m) = Macro average.\label{tab:results2}}
\end{table*}
